Multiscale Parareal Algorithm for Long-Time Mesoscopic Simulations of Microvascular Blood Flow in Zebrafish

Various biological processes such as transport of oxygen and nutrients, thrombus formation, vascular angiogenesis and remodeling are related to cellular/subcellular level biological processes, where mesoscopic simulations resolving detailed cell dynamics provide a key to understanding and identifying the cellular basis of disease. To break this bottleneck and achieve a biologically meaningful timescale, we propose a multiscale parareal algorithm in which a continuum-based solver supervises a mesoscopic simulation in the time-domain. Using an iterative prediction-correction strategy, the parallel-in-time mesoscopic simulation supervised by its continuum-based counterpart can converge fast. The effectiveness of the proposed method is first verified in a time-dependent flow with a sinusoidal flowrate through a Y-shaped bifurcation channel. Physical quantities of interest including velocity, wall shear stress and flowrate are computed to compare against those of reference solutions, showing a less than 1% relative error on flowrate in the Newtonian flow and a less than 3\% relative error in the non-Newtonian blood flow. The proposed method is then applied to a large-scale mesoscopic simulation of microvessel blood flow in a zebrafish hindbrain for temporal acceleration. The time-dependent blood flow from heartbeats in this realistic vascular network of zebrafish hindbrain is simulated using dissipative particle dynamics as the mesoscopic model, which is supervised by a one-dimensional blood flow model (continuum-based model) in multiple temporal sub-domains. The computational analysis shows that the resulting microvessel blood flow converges to the reference solution after only two iterations. The proposed method is suitable for long-time mesoscopic simulations with complex fluids and geometries.

==> comment.tex <==
{\color{red} XXX YH: THE SUPERSCRIPT OF $n$ and THE SUBSCRIPT OF $k$ NEED TO BE DEFINED CLEARLY IN THE TEXT. ALSO, $Q$ HAS NOT BEEN DEFINED ANYWHERE. XXX}

{\color{red}XXX YH: THE DEFINITION OF "CELL THICKNESS $h$" IS UNCLEAR. NEED TO SHOW WHICH LENGTH CORRESPONDS TO $h$ IN FIG.2 XXX}

{\color{red}XXX YH: THE ASSUMPTION OF "A PARABOLIC PROFILE" IS JUSTIFIED WHEN THE TIME PERIOD OF THE PULSATION IS SUFFICIENTLY LONGER THAN THE TIME SCALE DETERMINED BY THE FLUID VISCOSITY AND THE PIPE RADIUS. I ASSUME THIS CONDITION HOLDS HERE, BUT NEED TO BE POINTED OUT.XXX} 

{\color{red} XXX YH: DOES "spread" MEAN THE FLUCTUATION OF INSTANTANEOUS VELOCITY ? XXX}

{\color{red} XXX YH: WHAT ARE "TWO" SIMPLIFICATIONS ? ONLY NEWTONIAN ASSUMPTION IS WRITTEN ABOVE XXX}

{\color{red}XXX YH: THE WORD "TIMESTAMP" IS UNCLEAR. DOES IT MEAN THE TRAJECTORY OF EACH RBC CANNOT BE TRACKED BEYOND A CERTAIN SUBDOMAIN ? ANYWAY, IT IS BETTER TO UNIFY TERMINOLOGY THROUGHOUT THE TEXT. XXX}

{\color{red}XXX YH: I DO NOT UNDERSTAND WHAT THE ABOVE SENTENCE MEANS XXX.}

{\color{red}XXX YH: IN THE CASE OF EQ(2), THE VELOCITY PROFILE IS NOT MAINTINED, BUT A UNIFORM VELOCITY IS IMPOSED ACROSS THE CROSS SECTION IN FS, AM I CORRECT ? XXX}

==> intro.tex <==
The efficiency of the vascular network rests on the balance of two opposing requirements on network structures \cite{Secomb2013}. The demand for oxygen and nutrients necessitate a dense network, such that tissue cells are within the oxygen diffusion distance. A dense mesh-like network meets the requirement, but at the expense of high resistance to flow. Conversely, a tree-like network can minimize flow resistance but lacks uniform spatial coverage \cite{Secomb2013}. The actual vascular networks adapt a combination of mesh-like and tree-like networks to supply oxygen with approximately uniform density. Furthermore, it can remodel the existing network to adapt to new demands. Thus, vascular network formation is a complex problem of biological optimization \cite{Secomb2013} in disguise. 

Angiogenesis and pruning, along with vessel formation (vasculogenesis), are the main processes involved in vasculature formation. They are essential for biological functions including growth, wound healing and aging \cite{Zakrzewicz2015}. Angiogenesis is the process of new blood vessel formation from existing vascular structure \cite{Risau1997}. Vascular networks formed by sprouting angiogenesis subsequently undergo remodeling (\textit{e.g.} vascular pruning and regression of particular vascular branches) to form a mature and efficient vasculature \cite{Risau1997}. 

Aside from the desire to reveal nature’s design, a deep and thorough understanding of those processes also provide therapeutic value. As an indication of cancer and various ischaemic and inflammatory diseases, pathological angiogenesis provides new blood vessels needed to sustain abnormal growth, \textit{e.g.} tumors \cite{Carmeliet2011}. Vessel regression is an emerging field of research because of its therapeutic implications such as tumor inhibition. Further improvements will require a better understanding of angiogenesis and pruning.

Both angiogenesis and pruning were formerly understood as chemical driven processes. However, recent studies suggest that they are both mechanically and chemically driven \cite{Risau1997,Bernabeu2014,Huang2003}. Shear stress on vessel wall stimulates vessel regression through chemical signaling \cite{Franke1984,Resnick1995}, and is induced by red blood cell movements \cite{Xiong2010,Hogan2019,Oulaid2015}. A mechanically accurate model of blood with discrete red blood cells can accurately capture the effects of microcirculation on angiogenesis and pruning.

As an emerging model organism, zebrafish has many advantages over the traditional mouse model. Most notably, most vertebrate tissue of zebrafish larvae are transparent, which simplifies the examination of the vasculature \textit{in vivo}. Because of this, observations of angiogenesis and pruning, and the subsequent hypothesis proposal and testing are easily performed \cite{Chavez2016}. Furthermore, research has shown mutual translatability of findings between zebrafish and human vascular biology \cite{Coultas2005,Lieschke2007}. Thus, zebrafish as a tool to study human vasculature has been embraced by the community. 

Although discrete models of blood can capture complicated interactions between blood components and the vessel wall, it is costly to simulate such systems in practicality. An adult female zebrafish has a body length of 3.87 centimeters and an average blood volume of 17 microliters \cite{Zang2013}, which translates to $5.134\times10^{7}$ red blood cells \cite{Murtha}. A naive simulation (i.e. serial in time and space) with discrete red blood cells is unfeasible even for a sub-system that is $1\%$ of the volume. A typical strategy to accelerate a large-scale simulation is spatial decomposition, \textit{i.e.}, decompose the domain in space and then simulate all sub-domains concurrently with additional computing resources. This approach works very well for Lagrangian methods as they are highly parallelizable with good strong and weak scalings \cite{Blumers,Plimpton1995}. As a result, it has been incorporated into many well-known particle simulators \cite{Plimpton1995,Case2005,Pronk2013,Limbach2006,Smith1996}.

Besides the massive spatial coverage, a lengthy physical time scale is another bottleneck for Lagrangian particle simulations. Since the atomistic details are explicitly modeled, the maximum time step is limited by the smallest oscillation period of the fastest atomic motion, typically on the order of several femtoseconds \cite{Feenstra1999}. Consequently, the physical time scales accessible to those simulations are too short to address interesting long-time dynamics. In the example of thrombus formation caused by platelet margination and adhesion, the characteristic time for platelet activation is a few microseconds, and the formation processes usually require at least several hours to days \cite{Killer2010,Schriefl2012}. With a time step on the order of one microsecond, a clinically meaningful result for one-day time integration require $10^{11}$ time steps with the explicit platelet models \cite{Filipovic2008}, deeming it computationally prohibitive. To break the bottleneck, a supervised parallel-in-time algorithm for long-time Lagrangian simulations of stochastic dynamics (\AlgAbb{}) was proposed by Blumers et al \cite{Blumers2019}. Inspired by parareal \cite{Lions2001}, \AlgAbb{} is a predictor-corrector type algorithm for which the high-fidelity Lagrangian simulator (fine solver) is supervised by a low-fidelity continuum model (coarse solver). The results of the Lagrangian simulation then correct the mean-field prediction and provide the proper microscopic details (e.g., consistent fluctuations, correlations, etc.). 

In this work, we attempt to accelerate massive Lagrangian simulations of blood flow at mesoscale with application on zebrafish hindbrain. In addition, Spatial Decomposition (SD) method is applied in conjunction to additional speedup. The reminder of this paper is organized as follows: we first introduce \AlgAbb{} for the application of blood flow in section \ref{sec:solvers} and \ref{sec:SPASD}. We then explain in detail the coupling scheme in our implementation in section \ref{sec:multiframework}. Additionally, the section contains the software architecture that enables real-time data transfer in massive parallel simulations. In section \ref{sec:numericalresults}, we present quantitative results of simulations via our \AlgAbb{} framework. Finally, section \ref{sec:discussion} contains a brief summary and lengthy discussion. 
